Learning Key-Value Store Design

We introduce the concept of design continuums for the data layout of key-value stores. A design continuum unifies major distinct data structure designs under the same model. The critical insight and potential long-term impact is that such unifying models 1) render what we consider up to now as fundamentally different data structures to be seen as views of the very same overall design space, and 2) allow seeing new data structure designs with performance properties that are not feasible by existing designs. The core intuition behind the construction of design continuums is that all data structures arise from the very same set of fundamental design principles, i.e., a small set of data layout design concepts out of which we can synthesize any design that exists in the literature as well as new ones. We show how to construct, evaluate, and expand, design continuums and we also present the first continuum that unifies major data structure designs, i.e., B+tree, B-epsilon-tree, LSM-tree, and LSH-table. The practical benefit of a design continuum is that it creates a fast inference engine for the design of data structures. For example, we can predict near instantly how a specific design change in the underlying storage of a data system would affect performance, or reversely what would be the optimal data structure (from a given set of designs) given workload characteristics and a memory budget. In turn, these properties allow us to envision a new class of self-designing key-value stores with a substantially improved ability to adapt to workload and hardware changes by transitioning between drastically different data structure designs to assume a diverse set of performance properties at will.

==> build-figures.tex <==
% externalize to pdf
%
%%%%% NOTE: The Original Model Table
\pagebreak
\include{models}
\pagebreak

%%%%% NOTE: The Original Instances Table
\pagebreak
\include{design-instances-table}
\pagebreak

%%%%% NOTE: The LSH Extended Model Table
\pagebreak
\include{models-lsh-diff}
\pagebreak

%%%%% NOTE: The LSH Extended Instances Table
\pagebreak
\include{design-instances-table-lsh}
\pagebreak

==> design-instances-table-lsh.tex <==
%%%%%% NOTE: 
% Compile this first to PDF
% Then we include that generated PDF in the top.tex
% NOTE: this table has bibtex cite references, which need to align nimerically
%       when it is generated alongside top.tex
%       so remember to regen this everytime you change \cites 

% \usetikzlibrary{matrix}
% \usetikzlibrary{positioning}
% \usetikzlibrary{fit}
% \usetikzlibrary{calc}


\tikzset{
    %%% Super Table Style
    table/.style = {
        matrix of nodes,
        row sep=-\pgflinewidth,
        column sep=-\pgflinewidth,
        nodes={
            rectangle,
            draw=black,
            align=center
        }
    },
    zebra_rows/.style = {
        every even row/.style={
            nodes={fill=gray!20}
        }
    },
    left_most_symbol_bold/.style = {
        column 1/.style={
            nodes={font=\bfseries}
        }
    },
    black_header/.style = {
        row 1/.style={
            nodes={
                fill=black,
                text=white,
                font=\bfseries
            }
        }
    },
    tall_header/.style = {
        row 1/.style={
            nodes = {
                font=\bfseries,
                minimum size=7em,
                %align=flush left
            }
        },
    },
    border_toprule/.style = {
        execute at end cell={
            \draw [line cap=rect,#1] (\tikzmatrixname-\the\pgfmatrixcurrentrow-\the\pgfmatrixcurrentcolumn.north east) -- (\tikzmatrixname-\the\pgfmatrixcurrentrow-\the\pgfmatrixcurrentcolumn.north west);
        }
    },
    border_bottomrule/.style={%
        execute at end cell={%
            \draw [line cap=rect,#1] (\tikzmatrixname-\the\pgfmatrixcurrentrow-\the\pgfmatrixcurrentcolumn.south west) -- (\tikzmatrixname-\the\pgfmatrixcurrentrow-\the\pgfmatrixcurrentcolumn.south east);%
        }
    },
    deriv_cell/.style={
        nodes = {
            minimum size=2.0em
        }
    },
    cost_cell/.style={
        nodes = {
            minimum size=3.0em,
            text depth=0.0ex,
            text height=0.0ex
        }
    },
    update_costs_style/.style={
        % row 10/.style=cost_cell,
        row 11/.style=cost_cell,
        row 12/.style=cost_cell,
        row 13/.style=cost_cell,
        row 14/.style=cost_cell
    },
    zpl_costs_style/.style={
        % row 10/.style=cost_cell,
        row 14/.style=cost_cell,
        row 15/.style=cost_cell
    },
    pl_costs_style/.style={
        % row 10/.style=cost_cell,
        row 16/.style=cost_cell,
        row 17/.style=cost_cell
    },
    srl_costs_style/.style={
        % row 10/.style=cost_cell,
        row 18/.style=cost_cell,
        row 19/.style=cost_cell
    },
    lrl_costs_style/.style={
        % row 10/.style=cost_cell,
        row 20/.style=cost_cell,
        row 21/.style=cost_cell
    },
    instances_table/.style={ 
        table,
        tall_header,
        minimum size=4em,
        text depth=0.0ex,
        text height=0.0ex,
        update_costs_style,
        zpl_costs_style,
        pl_costs_style,
        srl_costs_style,
        lrl_costs_style,
        nodes in empty cells
    },
    term_bold_instances_table/.style={
        instances_table,
        left_most_symbol_bold
    },
    % two styles to help the diagonal first row first cell style
    diag text/.style={inner sep=0pt, font=\footnotesize},
    shorten/.style={shorten <=#1,shorten >=#1},
    block/.style={
      rectangle,
      draw=blue,
      thick,
      fill=blue!20,
      text width=5em,
      align=center,
      rounded corners,
      minimum size=2em
    }
}

% \tikz[diag text/.style={inner sep=0pt, font=\footnotesize},
%       shorten/.style={shorten <=#1,shorten >=#1}]{%
%         \node[below left, diag text] (def) {def};
%         \node[above right=2pt and -2pt, diag text] (abc) {abc};
%         \draw[shorten=4pt, very thin] (def.north west|-abc.north west) -- (def.south east-|abc.south east);}


% %%%%%%%%%%%%%%%% BEGIN INSTANCES TABLE LSH, Beps, B+ %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[t]
    % \begin{minipage}[c]{\textwidth}

    {\scalefont{0.7} 
        \begin{tikzpicture}
            \coordinate (afterheady) at (0, 7em);
            \node (ParamsLabel) [outer ysep=1em, inner ysep=0.0em, align=center, below=of afterheady, rotatebox/.style={text width=4.0em, minimum size=18.0em, text height=18.0em, align=center}] {\rotatebox{90}{\large Parameters}};
            \coordinate (labeloffset) at (-4.0em,-8em);
            \node (MetricsLabel) [outer ysep=5em, inner ysep=0.0em, align=center, below=of ParamsLabel, rotatebox/.style={text width=4.0em, minimum size=6em, text height=6.0em, align=center}]  {\rotatebox{90}{\large Metrics}};
            \node(box2) [] at ($(ParamsLabel.north east)!0.5!(MetricsLabel.south west)$) {};

            \matrix (CIDRSummaryModelParamsLSM) [
                right=of labeloffset,
                term_bold_instances_table, 
                text width=7.3em, 
                row 1/.style={minimum size=7.3em, font=\bfseries},
                row 7/.style={cost_cell, border_toprule=ultra thick},
                row 8/.style={cost_cell}, 
                row 9/.style={cost_cell},
                row 10/.style={cost_cell},
                row 11/.style={cost_cell},
                %row 13/.style={cost_cell},
            ]
            {
                %%% FIRST CELL FIRST COL
                \node[below left, diag text, minimum size=1.5em, text width=2.5em, draw=none, outer sep=1.0pt] (Terms) {\scriptsize \textbf{Terms}};
                \node[above right, diag text, minimum size=1.5em, text width=2.5em, draw=none, outer ysep=-1.pt, outer xsep=-3.5pt] (Designs) {\scriptsize \textbf{Designs}};
                %\draw[black] ($(Terms.north west)+(-0.17,0.35)$)  rectangle ($(Designs.south east)+(0.17,-0.35)$);
                %\node[anchor=mid] at ($0.5 * (Terms.north east) + (Terms.north east) - (Designs.south east)$) {};
                \node[](box) at ($(Terms.north east)!0.5!(Designs.south west)$) {};
                \draw[very thin] (box.north west) -- (box.south east);
                                        & Log                   &  LSH Table \cite{Sheehy2010, Chandramouli2018, SpotifySparkey, Rumble2014, Lim2014, Ahn2016, Wu2018}        &  Sorted Array    \\
                T (Growth Factor)        & $\frac{N \cdot E}{M_B}$         & $\frac{N \cdot E}{M_B}$                                                                           &  $\frac{N \cdot E}{M_B}$ \\
                K (Hot Merge Threshold)    & $T-1$                        &  $T-1$                                                                                             &  $1$                    \\
                Z (Cold Merge Threshold)   & $T-1$                        &  $T-1$                                                                                             &  $1$                    \\
                D  (Max. Node Size)     & $\frac{N}{B}$          &  $\frac{N}{B}$                                                                                                                   &  $\frac{N}{B}$    \\
                \bm{$M_{F}$} (Fence \& Filter Mem.)  & $ \frac{N \cdot F}{B}$         & $N \cdot F \cdot (1 + \frac{1}{B}) $                                                                                                       &  $ \frac{N \cdot F}{B}$ \\
                %%%%% COSTS:
                Update                   & $O(\frac{1}{B})$             & $O(\frac{1}{B})$                                                                                                  &  $O(\frac{N \cdot E}{M_B \cdot B})$        \\
                Zero Result Lookup       & $O(\frac{N \cdot E}{M_B})$                       & $O(0)$                                                                                                             &  $O(1)$                 \\
                Single Result Lookup     & $O(\frac{N \cdot E}{M_B})$                       & $O(1)$                                                                                                             &  $O(1)$                 \\
                Short Range Scan         & $O(\frac{N \cdot E}{M_B})$      & $O(\frac{N \cdot E}{M_B})$                                                                                                            &  $O(1)$       \\
                Long Range Scan          & $O(\frac{N \cdot E}{M_B} \cdot \frac{s}{B})$     & $O(\frac{N \cdot E}{M_B} \cdot \frac{s}{B})$                                                                                          &  $O(\frac{s}{B}) $         \\
                %%%%%% BEGIN COMMENTED OUT FOR CIDR SUBMIT %%%%%%
                % %Zero Result Pt Lookup (Seq Read)               & $O(\frac{N}{B} \cdot e^{-\frac{M_{BF}}{N}})$            &$O(D \cdot T \cdot e^{\frac{-M_{BF}}{N}})$                                       & $O(D \cdot e^{-\frac{M_{BF}}{N}})$                                     & $O(D \cdot e^{-\frac{M_{BF}}{N}})$                           & $O(D \cdot e^{-\frac{M_{BF}}{N}})$                       & &\\
                % Existing Lookup                               & $O(1 + T \cdot e^{\frac{-M_{BF}}{N}})$                                          & $O(1)$                                                                 & $O(1)$                                                       &$O(L)$                                          & $O(L)$                       &$O(L)$                                                                                                    & $O(L)$\\
                % %Existing Point Lookup (Seq Read)               &$O((1 + \frac{N}{B \cdot D} \cdot e^{-\frac{M_{BF}}{N}}) \cdot D)$ & $O((1 + T \cdot e^{\frac{-M_{BF}}{N}}) \cdot D)$                      & $O(D)$                                                                 & $O(D)$                                                       & $O(D)$                                                   & &\\
                % Short Scan                                    &$O(L \cdot T)$                                                                   & $O(1 + T \cdot (L-1))$                                               & $O(L)$                                                       &$O(L)$                                          & $O(L)$                       &$O(L)$                                                                                                    & $O(L)$\\
                % %Short Range Scan (Seq Read)                    &$O(\frac{N}{B})$                                         &$O(L \cdot T \cdot D)$                                                           & $O((1 + T \cdot (L - 1)) \cdot D)$                                     & $O(L \cdot D)$                                               & $O(D)$                                                   & &\\
                % Long Scan                                     &$O(T \cdot \frac{s}{B} \cdot (1 + \frac{1}{D}))$                                 & $O(\frac{s}{B} \cdot (1 + \frac{1}{D}))$                               &  $O(\frac{s}{B} \cdot (1 + \frac{1}{D}))$                   & $O(\frac{s}{B} \cdot (1 + \frac{1}{D}))$      & $O(\frac{s}{B} \cdot (1 + \frac{1}{D}))$  &$O(\frac{s}{B} \cdot (1 + \frac{1}{D}))$                                                                    & $O(\frac{s}{B} \cdot (1 + \frac{1}{D}))$ \\
                % %Long Range Scan (Seq Read)                     &$O(\frac{N}{B})$                                         &$O(\frac{T \cdot s}{B})$                                                         & $O(\frac{s}{B})$                                                       &  $O(\frac{s}{B})$                                            &  $O(\frac{s}{B})$                                        & &\\
                %%%%%% END COMMENTED OUT FOR CIDR SUBMIT %%%%%%
            };
        \end{tikzpicture}
    }
    % \caption{The extended design continuum allows an additional set of data structure instances to be expressed.}
    % \label{f:instanceslsh}

    % \end{minipage}
\end{figure}
%%%%%%%%%%%%%%% END TABLE LSM, Beps, B+ %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> design-instances-table.tex <==
%%%%%% NOTE: 
% Compile this first to PDF
% Then we include that generated PDF in the top.tex
% NOTE: this table has bibtex cite references, which need to align nimerically
%       when it is generated alongside top.tex
%       so remember to regen this everytime you change \cites 


\tikzset{
    %%% Super Table Style
    table/.style = {
        matrix of nodes,
        row sep=-\pgflinewidth,
        column sep=-\pgflinewidth,
        nodes={
            rectangle,
            draw=black,
            align=center
        }
    },
    zebra_rows/.style = {
        every even row/.style={
            nodes={fill=gray!20}
        }
    },
    left_most_symbol_bold/.style = {
        column 1/.style={
            nodes={text width=7em, font=\bfseries}
        }
    },
    black_header/.style = {
        row 1/.style={
            nodes={
                fill=black,
                text=white,
                font=\bfseries
            }
        }
    },
    tall_header/.style = {
        row 1/.style={
            nodes = {
                font=\bfseries,
                minimum size=5.6em,
                %align=flush left
            }
        }
    },
    border_toprule/.style = {
        execute at end cell={
            \draw [line cap=rect,#1] (\tikzmatrixname-\the\pgfmatrixcurrentrow-\the\pgfmatrixcurrentcolumn.north east) -- (\tikzmatrixname-\the\pgfmatrixcurrentrow-\the\pgfmatrixcurrentcolumn.north west);
        }
    },
    border_bottomrule/.style={%
        execute at end cell={%
            \draw [line cap=rect,#1] (\tikzmatrixname-\the\pgfmatrixcurrentrow-\the\pgfmatrixcurrentcolumn.south west) -- (\tikzmatrixname-\the\pgfmatrixcurrentrow-\the\pgfmatrixcurrentcolumn.south east);%
        }
    },
    deriv_cell/.style={
        nodes = {
            minimum size=2.0em
        }
    },
    cost_cell/.style={
        nodes = {
            minimum size=3.0em,
            text depth=0.0ex,
            text height=0.0ex
        }
    },
    update_costs_style/.style={
        % row 10/.style=cost_cell,
        row 11/.style=cost_cell,
        row 12/.style=cost_cell,
        row 13/.style=cost_cell,
        row 14/.style=cost_cell
    },
    zpl_costs_style/.style={
        % row 10/.style=cost_cell,
        row 14/.style=cost_cell,
        row 15/.style=cost_cell
    },
    pl_costs_style/.style={
        % row 10/.style=cost_cell,
        row 16/.style=cost_cell,
        row 17/.style=cost_cell
    },
    srl_costs_style/.style={
        % row 10/.style=cost_cell,
        row 18/.style=cost_cell,
        row 19/.style=cost_cell
    },
    lrl_costs_style/.style={
        % row 10/.style=cost_cell,
        row 20/.style=cost_cell,
        row 21/.style=cost_cell
    },
    instances_table/.style={ 
        table,
        tall_header,
        minimum size=3.5em,
        text depth=0.0ex,
        text height=0.0ex,
        update_costs_style,
        zpl_costs_style,
        pl_costs_style,
        srl_costs_style,
        lrl_costs_style,
        nodes in empty cells
    },
    term_bold_instances_table/.style={
        instances_table,
        left_most_symbol_bold
    },
    % two styles to help the diagonal first row first cell style
    diag text/.style={inner sep=0pt, font=\footnotesize},
    shorten/.style={shorten <=#1,shorten >=#1},
    block/.style={
      rectangle,
      draw=blue,
      thick,
      fill=blue!20,
      text width=5em,
      align=center,
      rounded corners,
      minimum size=2em
    }
}

% %%%%%%%%%%%%%%%% BEGIN MAIN INSTANCES TABLE LSM, Beps, B+ %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}[t]
    \centering
    % \begin{minipage}[c]{\textwidth}
    {\scalefont{0.7} 
        % \begin{tikzpicture}
        %     \matrix (SummaryModelParamsLabel) [] 
        %     {
        %         \node [draw, rotatebox/.style={minimum height=12.0em, text height=5.0em}] (ParamsLabel) {\rotatebox{90}{Parameters}};
        %         \node [draw, below=of ParamsLabel, rotatebox/.style={minimum height=10.0em, text height=5.0em}] (MetricsLabel) {\rotatebox{90}{Metrics}};  
        %     };    
        % \end{tikzpicture}
            \begin{tikzpicture}
                % TODO: 
                % increase the font size
                % exact spacing, padding, margins between two matrix structures
                % as well as positioning of the two side labels
                %
                %
                \coordinate (afterheady) at (0, 7em);
                \node (ParamsLabel) [outer ysep=1em, inner ysep=0.0em, align=center, below=of afterheady, rotatebox/.style={text width=4.0em, minimum size=18.0em, text height=18.0em, align=center}] {\rotatebox{90}{\large Parameters}};
                \coordinate (labeloffset) at (-4em, -8em);
                \node (MetricsLabel) [outer ysep=3.5em, inner ysep=0.0em, align=center, below=of ParamsLabel, rotatebox/.style={text width=4.0em, minimum size=6em, text height=6.0em, align=center}]  {\rotatebox{90}{\large Metrics}};
                \node(box2) [] at ($(ParamsLabel.north east)!0.5!(MetricsLabel.south west)$) {};
                %\draw[very thin] (box2.north west) -- (box2.south east);
                
                \matrix (CIDRSummaryModelParamsLSM) [
                    right=of labeloffset,
                    term_bold_instances_table, 
                    text width=7.3em, 
                    row 7/.style={cost_cell, border_toprule=ultra thick},
                    row 8/.style={cost_cell}, 
                    row 9/.style={cost_cell},
                    row 10/.style={cost_cell},
                    row 11/.style={cost_cell},
                    %row 13/.style={cost_cell},
                ]
                {
                    %%% FIRST CELL FIRST COL
                    \node[below left, diag text, minimum size=1.5em, text width=2.5em, draw=none, outer sep=1.0pt] (Terms) {\textbf{\scriptsize  Terms}};
                    \node[above right, diag text, minimum size=1.5em, text width=2.5em, draw=none, outer ysep=-1.pt, outer xsep=-3.5pt] (Designs) {\textbf{\scriptsize  Designs}};
                    %\draw[black] ($(Terms.north west)+(-0.17,0.35)$)  rectangle ($(Designs.south east)+(0.17,-0.35)$);
                    %\node[anchor=mid] at ($0.5 * (Terms.north east) + (Terms.north east) - (Designs.south east)$) {};
                    \node[](box) at ($(Terms.north east)!0.5!(Designs.south west)$) {};
                    \draw[very thin] (box.north west) -- (box.south east);
                                                                & Tiered LSM-Tree \cite{Lakshman2010,Dayan2017,Dayan2018a,Jagadish1997}           & Lazy Leveled LSM-Tree \cite{Dayan2018, Dayan2018a}                                 & Leveled LSM-Tree \cite{GoogleLevelDB,FacebookRocksDB,Dayan2017, Dayan2018a} &COLA \cite{Bender2007}            & FD-Tree \cite{Li2010}           &\bm{$B^\epsilon$}Tree \cite{Brodal2003, Bender2007, Jannen2015, Papagiannis2016, Arge2003, Jermaine2007}        & \bm{$B+$}Tree \cite{Bayer1970}  \\
                    T (Growth Factor)                             & $\lbrack 2,B \rbrack$                                                           & $\lbrack 2,B \rbrack$                                                  &$\lbrack 2,B \rbrack$                                        & 2                                            & $\lbrack 2,B \rbrack$           &$\lbrack 2,B \rbrack$                                                                                     & $B$ \\ %$B$ $\lbrack B, T \rbrack$ \\
                    K (Hot Merge Threshold)                         &  $T-1$                                                                          & $T-1$                                                                  & 1                                                            &1                                            &1                                &1                                                                                                         &1\\
                    Z (Cold Merge Threshold)                        &  $T-1$                                                                          & 1                                                                      & 1                                                            &1                                            &1                                &1                                                                                                          &1 \\
                    D (Max. Node Size)                          &  $\lbrack 1,\frac{N}{B} \rbrack$                                              & $\lbrack 1,\frac{N}{B} \rbrack$                                          & $\lbrack 1,\frac{N}{B} \rbrack$                           &$\frac{N}{B}$                                 & $\frac{N}{B}$                 &1                                                                                                          & 1\\
                    %bm{$M_{B}$}                                & $D \cdot B \cdot E$                                                             & $D \cdot B \cdot E$                                                      & $D \cdot B \cdot E$                                       &$D \cdot B \cdot E$                             &$D \cdot B \cdot E$              &$E \cdot D \cdot (B - T)$                                                                                  & 0 \\
                    %%%% CIDR SUBMISSION, FIX BUFER TO DBE. %%%%%
                    % \bm{$M_{B}$}                                & $D \cdot B \cdot E$                                                             & $D \cdot B \cdot E$                                                      & $D \cdot B \cdot E$                                       &$D \cdot B \cdot E$                             &$D \cdot B \cdot E$              &$B \cdot E$                                                                                  & $B \cdot E$ \\
                    % Collapsed M_{FP} and M_{BF} into one knob
                    %$M_{FP}$                                        & $F \cdot \frac{N}{B}$                                   & $F \cdot \frac{N}{B}$                                                           & $F \cdot \frac{N}{B}$                                                  & $F \cdot \frac{N}{B}$                                        & $F \cdot \frac{N}{B}$                                    &0 &0\\
                    %$M_{BF}$                                        & $10 \cdot N$                                            & $10 \cdot N$                                                                    & $10 \cdot N$                                                           & $10 \cdot N$                                                 & $10 \cdot N$                                             &0 &0\\
                    \bm{$M_{F}$} (Fence \& Filter Mem.)           & $N \cdot (\frac{F}{B} + 10)$                                              & $N \cdot (\frac{F}{B} + 10)$                                     & $N \cdot (\frac{F}{B} + 10)$                          &$\frac{F \cdot T \cdot M_B}{E \cdot B}$                                           &$\frac{F \cdot T \cdot M_B}{E \cdot B}$                            &$\frac{F \cdot T \cdot M_B}{E \cdot B}$                                                                                                          &$\frac{F \cdot T \cdot M_B}{E \cdot B}$ \\
                    %%%%%%%%% COSTS:
                    Update                                        & $O(\frac{L}{B})$                                                        & $O(\frac{1}{B} \cdot (T + L))$                                         & $O(\frac{T}{B} \cdot L)$                                  &$O(\frac{L}{B})$                               & $O(\frac{T}{B} \cdot L)$ &$O(\frac{T}{B} \cdot L)$                                              & $O(L)$ \\
                    Zero Result Lookup                            &$O(T \cdot e^{\frac{-M_{BF}}{N}})$                                               & $O(e^{-\frac{M_{BF}}{N}})$                                             & $O(e^{-\frac{M_{BF}}{N}})$                                   &$O(L)$                                        & $O(L)$                         &$O(L)$                                                                                                    & $O(L)$\\
                    %%%%%% BEGIN COMMENTED OUT FOR CIDR SUBMIT %%%%%%
                    % %Zero Result Pt Lookup (Seq Read)               & $O(\frac{N}{B} \cdot e^{-\frac{M_{BF}}{N}})$            &$O(D \cdot T \cdot e^{\frac{-M_{BF}}{N}})$                                       & $O(D \cdot e^{-\frac{M_{BF}}{N}})$                                     & $O(D \cdot e^{-\frac{M_{BF}}{N}})$                           & $O(D \cdot e^{-\frac{M_{BF}}{N}})$                       & &\\
                    Existing Lookup                               & $O(1 + T \cdot e^{\frac{-M_{BF}}{N}})$                                          & $O(1)$                                                                 & $O(1)$                                                       &$O(L)$                                          & $O(L)$                       &$O(L)$                                                                                                    & $O(L)$\\
                    % %Existing Point Lookup (Seq Read)               &$O((1 + \frac{N}{B \cdot D} \cdot e^{-\frac{M_{BF}}{N}}) \cdot D)$ & $O((1 + T \cdot e^{\frac{-M_{BF}}{N}}) \cdot D)$                      & $O(D)$                                                                 & $O(D)$                                                       & $O(D)$                                                   & &\\
                    Short Scan                                    &$O(L \cdot T)$                                                                   & $O(1 + T \cdot (L-1))$                                               & $O(L)$                                                       &$O(L)$                                          & $O(L)$                       &$O(L)$                                                                                                    & $O(L)$\\
                    % %Short Range Scan (Seq Read)                    &$O(\frac{N}{B})$                                         &$O(L \cdot T \cdot D)$                                                           & $O((1 + T \cdot (L - 1)) \cdot D)$                                     & $O(L \cdot D)$                                               & $O(D)$                                                   & &\\
                    Long Scan                                     &$O(T \cdot \frac{s}{B} )$                                 & $O(\frac{s}{B} )$                               &  $O(\frac{s}{B} )$                   & $O(\frac{s}{B} )$      & $O(\frac{s}{B} )$  & $O(\frac{s}{B} )$                                                                   & $O(\frac{s}{B} )$ \\
                    % %Long Range Scan (Seq Read)                     &$O(\frac{N}{B})$                                         &$O(\frac{T \cdot s}{B})$                                                         & $O(\frac{s}{B})$                                                       &  $O(\frac{s}{B})$                                            &  $O(\frac{s}{B})$                                        & &\\
                    %%%%%% END COMMENTED OUT FOR CIDR SUBMIT %%%%%%
                };      
            \end{tikzpicture}
    }
    % \caption{Instances of the design continuum and examples of their derived cost metrics.}
    % \label{f:instances}
    % \end{minipage}
\end{figure*}

%%%%%%%%%%%%%%%% END MAIN INSTANCES TABLE LSM, Beps, B+ %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> design.tex <==
% !TEX root = top.tex
\section{Data Continuums}

%%%%%%%%% BEGIN KV FIGURE %%%%%%%%%%%%%%%%%

\begin{figure*}[ht]
    \includegraphics[page=1, width=0.3\textwidth]{visuals/kv-concepts.pdf}
    \hspace{0.05\textwidth}
    \includegraphics[page=1, width=0.6\textwidth]{visuals/kv-detailed.pdf}
    \caption{Key-Value Storage Engine Design Model reasons about how access patterns navigate across memory and disk-resident data.}
\end{figure*}

%%%%%%%%% END KV FIGURE %%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%% IMPORT DESIGN INSTANCE TABLE  %%%%%%%
\include{design-instances-table}

\begin{figure*}[ht]
    \includegraphics[page=1, width=0.95\textwidth]{tables/ModelCombinedTable.pdf}
    \includegraphics[page=1, width=0.95\textwidth]{visuals/Spectrums.pdf}
\end{figure*}


%%%%%%%%%%%% BEGIN Algorithm %%%%%%%%%%%%
\SetKwProg{update}{Update}{}{}
\SetKwProg{pointlookup}{PointLookup}{}{}


% For comments use tcp{} and tcc{}

\begin{algorithm}
	\update{(entry)}{
		\scriptsize

		\tcp{When a level must overflow to the next, there will be a run to flush}
		$runToFlush := NULL$\;
	
		% Buffer 
		\eIf{$M_{BUF} > E$}{ %\tcp{buffer is enabled}
			buffer.add($entry$)\;
			%buffer.add(entry)\;
			\If{buffer.numEntries $\geq B \cdot D$}{ %\tcp{buffer is full}
				$runToFlush := $Run(buffer)\; %\tcp{empty buffer and flush contents as a run}
			}
		}{
			$runToFlush := $Run(entry) \; %\tcp{no buffer enabled, flush one entry as a run}
		}

		\For{$i\gets0$ \KwTo $L$}{
            $levels$[$i$].runs.push($runToFlush$)\;
            \tcp{vary run merge rate for hot/cold levels}
			$numRunsAllowed$ := $i < (L-Y)$ ? $K : Z$\;
			\If{$levels$[$i$].runs.count $\geq numRunsAllowed$}{
				$levels$[$i$].runs := merge($levels$[$i$].runs, $runToFlush$)\; %\tcp{Conduct Horizontal Merge of runs at level $i$}

				\eIf{$levels$[$i$].capacity $\geq T^{i}$}{
					$runToFlush$ := level.runs.pop()\; \tcp{flush oldest run to next level}
				}{
					\textbf{return}\; %\tcp{No more merging necessary, abort.}
				}
			}
		}
	}
	\caption{In the update algorithm, merge frequency switches between hot and cold data levels in storage.}
	\label{algo:update}
\end{algorithm}



\begin{algorithm} 
	%\underline{\textbf{Autotune($N, E, \alpha, \phi, \Omega), $} }\\ 
	\pointlookup{($searchKey$)}{
		\scriptsize
		%	\KwData{this text}
		%	\KwResult{how to write algorithm with \LaTeX2e }
		
		% search buffer for the entry. stop if found
		\If{$M_{BUF} > E$}{ %\tcp{buffer is enabled}
			entry := $buffer$.find($searchKey$)\;
			\If{entry}{
				\textbf{return} \textit{entry};
			}
			%%% NOTE: explicit writing out, parse two entry opcode cases to entry, or entry DNE
			% entry := buffer.find($searchKey$)\;
			% %buffer.add(entry)\;
			% \If{entry}{
			% 	\If{eentry.op == insert}{ %\tcp{buffer is full}
			% 		\textbf{return} \textit{entry}; 
			% 	}
			% 	\textbf{return} \textit{doesNotExist}
			% }
		}
		\tcp{Direct page access to root node.}
		$pageToCheck$ := $levels$[0].runs[0].nodes[0]\;

		\For{$i\gets0$ \KwTo $L$}{
			% $isHotLevel$ := $i < (L-Y)$\;
			% $isFirstColdLevel$ := $i == (L-Y)$\;
			\For{$j\gets0$ \KwTo $levels$[$i$].runs.count}{
				\tcc{Prune search using bloom filters and fences when available.}
				\uIf{$i < (L-Y)$ \tcp{At hot levels.}}{
					$keyExists$ := $bloomFilters$[$i$][$j$].checkExists($searchKey$)\;
					\eIf{$!keyExists$}{
						\textbf{continue};
					}{
						$pageToCheck$ := $fences$[$i$][$j$].find($searchKey$)\;
					}
				}
				\ElseIf{$i == (L-Y)$ \tcp{At first cold level.}}{
					$pageToCheck$ := $fences$[$i$][$j$].find($searchKey$)\;
				}

				%\If{$pageToCheck$}{
					$entry$, $pageToCheck$ := pageToCheck.find($searchKey$)\;
					\If{$entry$}{
						\textbf{return} \textit{$entry$};
					}
				%}
			}
		}
		\textbf{return} \textit{$keyDoesNotExist$};
	}
	\caption{Point lookup uses in-memory bloom filters and fences to prune and direct search when possible, after which node navigation is done via embedded cascading fences.}
	\label{algo:pointlookup}
\end{algorithm}

%%%%%%%%%%%% END Algorithm %%%%%%%%%%%%



%%%%%%%%%%%%% BEGIN bl rough text %%%%%%%%%%%%%%%%%%
\paragraph{Adjustments to parameters.}
With a combined memory budget for fence pointers and bloom filters, we expose $M_{FPBF}$
which allocates memory to a stucture in the following process.
First, we proceed by level starting from the top of the data structure. 
For each level, we allocate first to $M_{FP}$, fence pointers.
We then allocate $M_{BF} = X$, for bloom filters.

$M = M_{BUF} + M_{FPBF} = M_{BUF} + M_{FP} + M_{BF}$.


\subsection{Parameter Tuning Intuition}

We briefly discuss each model parameter's tuning range of allowed minimum and maximum values, 
and the corresponding data structure design intuition. 

\paragraph{D: Node Size}

$D$ defines the size of a node, which is the unit of contiguous data region.
Therefore, varying $D$ dictates the fragmentation of the data layout on disk.
$D$ = 1 relaxes the fragmentation to many page-sized nodes, 
while $D = \frac{N}{B}$ enforces that the entire dataset is contiguously contained
as a single large node.

\paragraph{$M_{BUF}$: Write Buffer Memory Budget}

$M_{BUF}$ defines the amount of main memory allocated for the purpose
of amortizing the cost of integrating groups of new entries with the portion of the data
structure already on-disk; 
new writes are effectively cached in the write buffer until they are flushed
to the larger part of the data structure.

This knob dictates how many nodes worth of writes can be contained in the write buffer. 
At its smallest, the write buffer supports $D$ pages in-memory, the size of one node. 
At most, the write buffer could contain the entire dataset.

We note that functionally, data entries residing in the write buffer is equivalent to
a buffer pool for caching new data with a LRU policy for flushing the buffer.

ASSUMPTION: there is an assumption that the write buffer flushes entirely once full,
sending its full capacity of new entries to the on-disk portion of the data structure.

\paragraph{$M_{FPBF}$: Combined Fence Pointer and Bloom Filter Memory Budget}
The BL-model assumes a range of memory options for the combined fence pointer
and bloom filter budget.
$M_{FPBF} = M_{FP} + M_{BF}$.
The BL-model assumes memory is assigned to $M_{FP}$ internally first,
up to a density of 1 fence per page (B entries).
Any remaining $M_{FPBF} - M_{FP} = M_{BF}$ is assigned to bloom filters.
See Monkey assumptions about bloom filters TODO.

\paragraph{$M_{FP}$: Fence Pointer Memory Budget}

$M_{FP}$ defines the amount of main memory allocated to hold fence pointers in-memory for direct access.
In-memory fences are held soley in a form external to the node.
Fence pointers that cannot use this budget, must exist solely in-node in cascading fence pointer (CFP) form.

This knob controls how many fence pointers we can keep purely in-memory,
determined by starting from the fences of the root node, and navigating down the data structure depth 
level by level until the budget threshold is reached.
Deeper levels that exist beyond the threshold, keep fence pointers in-node.

$M_{FP}$ = 0 indicates that all fence pointers exist in-node only and are not kept in a dedicated main memory fence pointer pool. 
At the other extreme, $M_{FP} = F \cdot N/B$ indicates all fence pointers are kept in-memory, 
much like in the ideal LSM condition.

An assumption is that higher/shallower fence pointers are preferable to keep in memory, 
while lower/deeper fence pointers are best kept on-disk as fence pointers that cascade from node to node. 

\paragraph{$M_{BF}$: Bloom Filter Memory Budget}

$M_{BF}$ defines the amount of main memory allocated for the purpose of
holding bloom filters in-memory for pruning unnecessary node accesses during
query processing.

This knob constrains the total cumulative memory that bloom filters can occupy,
however, this knob does not dictate how this memory budget is
assigned to individual bloom filters.
Bloom filters could be assigned in a variety of policies: e.g. 
per node at the largest level, per level, per entire data structure.

$M_{BF}$ = 0 indicates no bloom filters are enabled anywhere in the data structure. 
At the other extreme, as $M_{BF}$ approaches $N \cdot F$, 
the bloom filter space usage resembles using memory to cache full length keys,
to be used as a set membership test with guaranteed zero false positive rate. 
use the $N \cdot F$  

\paragraph{T: Size Ratio}

$T$ is the ratio expressing capacity of a level $L$ with respect to that of its preceding level $L-1$. 
When a given level exceeds its allowed size ratio $T$, 
then a compaction needs to occur inter-level 
(a node will be vertically moved from the current level $L$ to the next deeper level $L+1$).

$T$ directly determines the depth (number of levels) in a data structure.
L, the data structure depth is obtained by $L = \log_{T}{\frac{N}{B \cdot D}}$.
$T = 2$ enforces the deepest hierarchical structure - 
(when there is no fence pointer memory budget, the resulting data structure resembles a buffered repository tree).
$T=\frac{N}{B \cdot D}$ enforces the flattest structure - resembling a single level data structure. 

This is also commonly referred to as the fanout in $B^\epsilon$ trees,
for which it is at most $B$ or $B-1$ (depending on implementation) under the maximum fanout of the Block Access Model. 

\paragraph{K: Merge Greediness (all but last level)}

$K$ controls merge greediness at all levels except the last level of the data structure.
When a level hits the threshold of $K$ number of runs, 
an intra-level compaction must occur (horizontal merge of adjacent runs at the same level).
$K$ determines the shape of individual levels expressed in grouping of runs. 

For K = $1$, the data structure levels maintain a layout of a single run behaving as a sorted array. 
For K = $T-1$, each level layout maintains a group of up to $T-1$ runs behaving as a log.

\paragraph{Z: Merge Greediness (last level)}

$Z$ controls for merge greediness at the last level of the data structure.
In effect, $Z$ is a specialized instance of $K$ parameter for the last level.
At Z=1, the last level resembles a contiguous sorted array. 
As Z increases, it resembles more and more of a log.

\subsection{Model Objectives}
The $BL-Tree$ model exposes a set of data structure design parameters.
These parameters dictate the shape and layout of a data structure,
and specify main memory budgets to features that accelerate query processing.

The tuning of these seven parameter knobs work in conjunction with
some strong assumptions about how aspects of the supporting
data access algorithms must work. 

However, these knob tunings also leave degrees of freedom for 
HOW to implement data access algorithms.

For instance, while the three memory budget knobs 
are bound by the invariant $M = M_{BUF} + M_{FP} + M_{BF}$, 
and define an available memory assignment between the three categories
of Buffer, Fences, and Bloom Filters, it does not necessarily tell us how 
to use use these budgets within each category.

Our model does not specify an explicit strategy for where in the
data structure to maintain bloom filters.

Our model fixes a simple strategy for assigning the fences memory budget
based on data structure depth, prioritizing holding the fences of more recent nodes in memory.
Loosening this assumption is also possible,
to include other strategies for determining which fences are held in memory.

Likewise, we fix an assumed pattern for moving data contents
from the write buffer between memory and disk,
with complete flushes of the write buffer.


\subsection{Generalized Cost Model}

In the following generalized BL cost model, 
we provide the asymptotic cost summaries of common query execution types.
We separate the costs into random and sequential components.
Reads are accounted in number of random probes to disk, and 
additional contiguous regions longer than 1 page are scanned are counted as additional sequential pages read.
Writes are accounted in number of pages written to disk (sequential writes).

\subsubsection{$M_{FPBF}$: Memory threshold}
$Y$ represents the number of levels in $B^\epsilon$-tree part of the data structure.
$Y$ can fall in one of three conditions depending on the budget of $M_{FPBF}$.
In the first condition there is sufficient memory budget for sufficient bloom filters and all fence pointers required,
at all $L$ levels, thus $Y = L$ in this case.
In the second condition there is enough memory budget for some levels to be in the LSM style, so $0 < Y < L$.
Level memory budgets are allocated on a per level basis starting from the top of the structure,
with $X + \frac{F}{B}$ bits assigned per entry, until the budget runs out.

In the third condition, there is less memory budget available than the memory required for the Fence Pointers
and Bloom Filters of a single node. In this case, the portion of the data structure that follows
LSM layout is non-existent, and the entirety of the structure follows $B^\epsilon$ navigation.
We show this by solving for $M_{FPBF}$ when $Y = L = \log_{T}{\frac{N}{B \cdot D}}$.


\begin{align*}
    Y =
    \left\{
        \begin{array}{ll}
            0  & \mbox{if } M_{FPBF} \geq N \cdot (X + \frac{F}{B})  \\
            \lfloor \log_{T}{\frac{N}{M_{FPBF}} \cdot \lparen X + \frac{F}{B} \rparen } \rfloor & \mbox{if } B \cdot D \cdot (X + \frac{F}{B}) < M_{FPBF} < N \cdot (X + \frac{F}{B}) \\
            L & \mbox{if } M_{FPBF} < B \cdot D \cdot (X + \frac{F}{B})
        \end{array}
    \right.
\end{align*}



\subsection{LSM}

\subsubsection{Logs}
Write-optmized key-value stores often take a log approach to data management.
We see this in recent log systems and tunings of LSM-based systems \cite{Lakshman2010,GoogleLevelDB,FacebookRocksDB,Dayan2017,Dayan2018}.

Log Structured Merge structures have an effective optimization for amortizing write I/O costs
on update operations.
By batching writes from memory to disk, new updates are accumulated in an in-memory buffer pool
and all updates flush from the buffer once full.
Entries may represent operations of setting an new key to a new value,
overwriting an old key to a new value,
or deleting an old key value pair.
Allocating a budget of $M_{BUF} = D \cdot B \cdot E$ bits for the in-memory buffer pool
allows the buffer pool to comfortably flush its content
in sorted form to a same-sized file on immutable disk. 
This immutable file is the smallest contiguous unit of disk-write, 
commonly known as a SSTable for many LSM-based key-value systems \cite{GoogleLevelDB,FacebookRocksDB}.
Note that each file is one-to-one correspondent to our BL-model node.
Thus a node is size $D$ contiguous pages holding $B$ entries per page, with $E$ bits per entry.

Typical LSM systems maintain main memory budgets also for fences and bloom filters
to help read accesses.
With a typical fence pointer memory budget of $M_{FP} = F \cdot \frac{N}{B}$,
there is enough memory to guarantee that all nodes have a fence per page kept in-memory.
Note the assumption that there is no need 
to budget more than just one fence per page.

For a bloom filter memory budget of $M_{BF} = 10 \cdot N$,
there is enough to guarantee 10 bits of bloom filter space
per entry of data. 
This is typcial for many standard LSM-based systems.
[Citation?].

The depth of a LSM-Tree is determined by $T$, the size ratio
between adjacent levels.
For instance, logs are single level structures,
becuase they have a size ratio of $T = \frac{N}{B \cdot D}$.
This makes the depth $L = 1$,
meaning the complete dataset is held in the only level of the data structure.

LSM-Trees can hold up to $K$ runs of data per level, and up to $Z$ runs at the last level.
Thus, for logs, 
they are a single level data structure 
that allows as many runs as there are nodes (effectively each node written to persistent storage is a run), 
so $K = T-1$, $Z = T-1$.
[TODO: Need to clarify difference between K, Z here?].

The update cost derives from one flush of the in-memory update buffer.
Each time the buffer flushes, one node of $D$ pages
is written to disk. 
On average, for each level, this results in $\frac{1}{B \cdot D}$ random writes per entry and 
$\frac{1}{B}$ sequential page writes per entry.
Because the log is a single level data structure, the multiplicative factor is just $L=1$.
Consider that an entry is written to disk only once and 
the log does do future merges of immutable nodes.

The point lookup cost derives from the search of the entire log,
aided by available bloom filters and in-memory fence per page of data.
Since there are $\frac{N}{B \cdot D}$ nodes in the data structure,
each node has to be pruned during search.

Therefore, a zero-result point lookup looking for a non-existent key
has $\frac{N}{B \cdot D}$ nodes to search through
and a $e^{-\frac{M_{BF}}{N}}$ probability of each node's bloom filter check returning a false positive
for the desired key to exist there.
We arrive at this false positive rate effect on search,
because we can reason about the behavior of many smaller bloom filters each at the node scope 
having similar asymptotic false positive rates as the same memory being allocated 
to a large bloom filter at the level scope \cite{Tarkoma2012}.

Accordingly a point lookup of an existing key has the same false positive cost component, in addition to one 
page where the desired key exists which needs to be searched.

A short range lookup for a LSM-Tree potentially 
must check one node per run.
However, since the log is only one level, with as many runs as nodes, it has to search every node,
since bloom filters cannot be leveraged to prune range lookups.

A long range lookup for a LSM-Tree must also scan an amount of all runs proportional 
to the scan selectivity. 
However, because the log is composed of single node runs,
each run must be scanned, resulting in asymptotic search cost of all nodes being touched.

\label{sec:design}




==> transitions.tex <==
\section{Transitions to Self-design}
Knowing which design is the best for a specific workload opens the opportunity for systems that can adapt on-the-fly by transitioning among different designs. As in all adaptive studies, we need to consider the benefit and the cost of the transition. The new challenge here is that such systems would transition among fundamentally different designs and ideally we would like to avoid reading and writing all data. In this section, we do a first discussion to demonstrate that it is possible to transition among what we normally consider as fundamentally different designs. Specifically we use the example of Leveled LSM-tree and B$^{+}$tree in our design continuum. 

In all of these cases, we represent our B$^{+}$Tree by storing only the leaf nodes on disk and the intermediate nodes in memory. $N$ stands for the total size of data in bytes, $p$ for size of each page, $s_0$ for the size of the buffer, T for the size ratio, and $\phi$ stands for the ratio of write to read cost.

\textbf{Lazy Transition: Wait for One Run.} 
One way to do such a transition is to wait until the LSM-tree is in a state where all of the entries are at the bottom level and then build the B$^{+}$Tree off of that level so that we don't have to copy the data (similar to how we build the internal index of B$^{+}$tree when we do bulk loading). We need to read the $\frac{N}{p}$ pages in the bottom level of the LSM-tree and subsequently create the B$^{+}$Tree index in main memory. Future updates to the B$^{+}$tree will require at most 1 page read and 2 page writes (in the case of splitting leaves), giving an upper bound to cost of $(1 + 2\phi)$ per update. (We avoid inducing a fill factor during the transition as that would mean reading and writing all leaf data.)

\textbf{Aggressive Transition: Preemptive Merging.}  
A second option is to preemptively merge the levels of the LSM-tree into a single level so we can build the B$^{+}$Tree off of that level without waiting for a natural merge to arrive. Assume, the $i$th level has size $s_0 T^i$. We have to read all of the pages from all of the levels, so the total number of disk reads forms a geometric series:
\[ \text{Pages Read} = \sum_{i=1}^{L} \frac{s_0 T^i}{p} = \frac{s_0(T^{L + 1} - 1)}{p(T-1)} \]
To write all of the entries to disk, we multiply this by $\phi$:
\[ \text{Write Cost} = \frac{\phi s_0(T^{L + 1} - 1)}{p(T-1)} \]
\[ \text{Worst Case Cost} = \frac{s_0(1 + \phi)(T^L - 1)}{p(T-1)} \]

Now we look at the general case where each level can have an arbitrary number of keys.  In order to calculate the cost, we let $x_i$ be the size of level $i$ in terms of bytes.  In this case we can compute the number of disk pages that our data takes up by computing the sum of disk pages in each level.  We then have to read and write this number of pages, so we multiply this sum by a factor of $(1 + \phi)$:
\[ \text{Cost} = \left( \sum_{i=1}^L \left\lceil \frac{x_i}{p} \right\rceil \right) (1 + \phi) \]

As we write this sorted array, we construct the intermediate nodes of the B$^{+}$tree in memory.

\textbf{Transitioning from arbitrary LSM-tree states.}
A third option is a compromise between the two: we use the bottom level of the LSM-tree as the leaf layer of the B$^{+}$Tree (avoiding copying the data) and then insert entries from the smaller levels of the B$^{+}$Tree into the LSM-Tree one by one. Below we analyze and determine I/O costs for each of these cases.  We now construct the cost such a hybrid transition algorithm which effectively includes the cost to build the index of a B$^{+}$tree for the last level of the LSM-tree plus the cost to gradually insert the remaining entries. 
\begin{align*}
    \text{Cost} &= \left\lceil \frac{x_L}{p} \right\rceil +  \sum_{i=1}^{L-1} \left( \frac{x_i}{p} + x_i(1 + 2\phi) \right) 
    %&= \left\lceil \frac{x_L}{p} \right\rceil +  \sum_{i=1}^{L-1} x_i \left( \frac{1}{p} + 1 +  2\phi \right)
    % &= \left\lceil \frac{x_L}{p} \right\rceil + \left( \sum_{i=1}^{L-1} x_i \right)(\frac{1}{p} + \phi)
\end{align*}

% An alternative option here is to preemptively merge only some of the LSM-tree levels, e.g., say we merge the lowest $k$ levels. To find the worst case cost, we assume that inserts into the B$^{+}$Tree always cause a split.  This leads to the following transition cost:
% \[ \text{Cost} = \sum_{i=L-k+1}^L \left\lceil \frac{x_i}{p} \right\rceil (1 + \phi) + \sum_{i=1}^{L-k} x_i \left( \frac{1}{p} + 1 +  2\phi \right) \]
% From looking at this equation, we can tell that the optimal $k$ is $k = L$ because it is cheaper for each entry to be part of the merge process than it is to be inserted into the B-tree.  Thus, this method is not useful but helps in our discussion.  It shows that if we preemptively merge any levels to make a B-tree, it is optimal to merge all levels at once.  

% Question: Are there better bounds we can get with bulk insert? In particular, we are inserting sorted runs. Also, the $2\phi$ bound is worst case. Is that ok?

\textbf{Adaptively Choosing how to Transition.}
When comparing all transition strategies, we observe that it is always better to preemptively merge than to wait. The intuition is that the last merge when waiting, reads and writes all data, which has the same I/O cost as preemptively merging.  Moreover, while waiting for the merge to occur naturally, the system is locked in a sub-optimal performance balance (assuming the target design is the best one for the current workload). 

This leaves us with the other two transition methods to choose from which leads to the following inequality
\[ \left\lceil \frac{x_L}{p} \right\rceil +  \sum_{i=1}^{L-1} x_i \left( \frac{1}{p} + 1 +  2\phi \right) < \left( \sum_{i=1}^L \left\lceil \frac{x_i}{p} \right\rceil \right) (1 + \phi) \]
\[ \to \sum_{i=1}^{L-1} x_i \left( 1 + 2\phi \right) < \left( \sum_{i=1}^L \left\lceil \frac{x_i}{p} \right\rceil \right) \phi \]
\[ \to x_L > \frac{p}{\phi} \sum_{i=1}^{L-1} x_i \left(1 - \frac{\phi}{p} + 2\phi \right) \]

The intuitive explanation of this inequality is that if the LSM-Tree is "bottom heavy," it is better to use the bottom level as the B$^{+}$Tree leaves and incrementally insert the remaining entries from the upper levels of the LSM-tree.  Otherwise, if it is ``top heavy," it is better to preemptively merge to create a single run and build the B$^{+}$Tree index from there.  

\textbf{Towards a Transition Algebra.} We omit several other possible options here due to space restrictions. The opposite transition is also possible from an B$^{+}$Tree to an LSM-tree with the opposite problem that the scattered leaves of the B$^{+}$Tree now needs to represent a contiguous run in an LSM-tree. To avoid a full write in this case we can trick virtual memory to consider these pages as contiguous using the RUMA method \cite{Schuhknecht2016}. The very first time the new LSM-tree does a full merge, the state would go back to actually physically contiguous runs. Overall, this very first exposition of possible transitions in this section, shows that it is possible to actually do such transitions at a smaller cost than reading and writing all data even if we transition among fundamentally different structures. The future path for a realization of this vision requires a full transition algebra.   

% We discuss how to estimate the waiting time for (3) in a later section.  

% \subsection{B-Tree to LSM-Tree}

% In this scenario, we want to transition from a B-Tree to an LSM Tree.  Let $X$ be the number of leaf nodes in our B-tree, and we assume that each leaf node takes up one disk page.  We also assume that leaf nodes are required to be at least half full.  This means that the number of disk pages represented by the leaf level of the B-tree is at most $X \leq \frac{2N}{p}$.  

% To do this transition, we propose two methods of taking the data from our B-tree and merging it into a single level of an LSM tree.  The first method is an eager merge where we immediately merge the leaf nodes, and the other is a lazy merge where we wait for the natural merge operation of the LSM tree until we merge the leaf nodes.  With either merge procedure, we need to generate the fence pointers for our resulting level.  We do this by scanning across the lowest intermediate level of our B-tree and merging the pointers so that we have a sorted, dense array of fence pointers in memory.  This is good because it is exactly the same format as a regular LSM tree's fence pointers, so it can be used to make our transition algorithm easy to integrate in existing LSM tree systems, as well as making it easy to modify and maintain.  We can also free the higher intermediate levels from our B-tree, freeing up some memory.  We may or may not choose not to generate a bloom filter from the leaf level of the B-tree, depending on the scenario (this is discussed below).

% \textbf{Method 1: Eager Merge.}
% With this method, we first scan the leaf level of the B-tree and re-write it as a dense, sorted array.  We use this dense array as the lowest level of our LSM tree, and this completes the transition.  The cost of this operation, in terms of disk IO is:
% \[ C(\text{transition}) = X + \phi \frac{N}{p} \leq \frac{2N}{p} + \phi \frac{N}{p} = \frac{N(2+\phi)}{p} \]
% This shows that the upper bound of the cost of this transition is $\frac{N(2+\phi)}{p}$.  This is a useful method because it allows the range queries of the resulting LSM tree to be fast as the lowest level is a dense sorted array (optimal for range queries).  While the cost of this transition is somewhat high, it is an immediate cost and may be useful if we wish to transition this data structure offline.  Because we are scanning all of the data anyway, we have the option of generating a bloom filter for this level in the LSM tree with no added disk IO cost.  We make this decision based off of the size of our data and our memory requirements, as it is possible that the data is so large that generating a bloom filter with a low false positive rate would use too much memory.  

% \textbf{Method 2: Lazy Merge.}
% In this method, we maintain the B-Tree as the bottom run of our LSM tree. As updates come in, we fill in the upper runs of our LSM tree, as usual. We will merge all the leaves of the B-Tree lazily when the above runs of the lsm tree are full.

% The cost of the transition happens during the lazy merge. The extra cost is in the reads during this merge (leaves may have some spaces):

% \[ C(\text{transition}) = X - \frac{N}{p} \]

% During the period in which the B-tree run has not been merged, we can cost different operations as compared with having a dense, sorted run. Inserts will have the same cost as the standard LSM tree (the merging of the B-tree run is accounted for in the transition cost). Range queries will have at most $2$ times as many disk accesses since leaf pages can be half full. If not bloom filter is created for the B-tree, point lookups will access $1$ disk page if the element is, regardless of whether the key is present. If a bloom filter is generated ($X$ disk reads overhead), then the expect number of page accesses when the key is not present is the false positive rate of the bloom filter.

% Question: Wouldn't range queries on B-trees be affected by the random accesses? Should this be incorporated into the model? Should we incorporate number of pages per leave?

% \subsection{Leveled LSM Tree to B-Tree: Average Case Analysis}

% Recall that in our transition from an LSM Tree to a B-Tree, we choose between two methods: either we take the bottom level of the LSM Tree and use it as the leaf nodes of the B-Tree (without copying the data), or we read all of the LSM Tree's values and merge them into a single sorted array, using that as the B-Tree's leaf level.  In our previous document, we analyzed the worst-case cost of both methods.  In this section, we look at a more average case for these transition algorithms.

% \begin{center}
% \begin{tabular}{|c|c|c|}
%     \hline
%     Symbol & Description & Unit \\
%     \hline
%     $\phi$ & Ratio of write cost to read cost & \\
%     $p$ & Page size & bytes \\
%     $N$ & Total size of data & bytes \\
%     $x_i$ & Amount of data in $i$th level of LSM Tree & bytes \\
%     $x_{-L}$ & Amount of data in all levels except $L$ & bytes \\
%     $\gamma$ & Proportion of entries in $x_{-L}$ that will cause a split when inserted into B-Tree & \\
%     $\alpha$ & Proportion of non-redundant entries in $x_{-L}$ & \\
%     $L$ & Number of levels in LSM Tree & \\
%     $u$ & Number of insert updates to LSM Tree per step & \\
%     $M$ & Number of steps in our transition & \\
%     \hline
% \end{tabular}
% \end{center}

% \textbf{Building From Lowest Level of LSM.}
% One way to look at the average case of this method is to assume that a proportion $\gamma$ of the entries in the upper levels of the LSM Tree will cause a split in the resulting B-Tree.  To simplify our cost expressions, let $x_{-L} = \sum_{k=1}^{L-1} x_k$ be the number of entries in the upper levels.  Thus, for each of the $x_{-L}$ upper entries, we need to first read this entry from the LSM tree run (with cost $\frac{1}{P}$), then we read the B-Tree leaf node (a cost of 1) and then insert it into the B-Tree leaf node, which will have an average write cost of $\gamma 2 \phi + (1 - \gamma)\phi$.  We also need to read into memory all of the pages in the lowest level of the LSM tree, which we do with cost $\left\lceil \frac{x_L}{p} \right\rceil$.  Putting this together, we get the following cost expression:
% \[ \text{Cost} = x_{-L}\left( \frac{1}{p} + 1 + \gamma 2 \phi + (1 - \gamma)\phi \right) + \left\lceil \frac{x_L}{p} \right\rceil \]
% This is a simple expression to compute and our only assumption was that a proportion $\gamma$ of our incremental B-Tree updates would cause a split.  However, the $\gamma$ parameter is not easy to predict - we could either attempt to estimate it by making assumptions about the distribution of the updates or simply use a constant to estimate this cost.  

% We consider the expected cost of B-tree inserts  when the $L - 1$ levels form a uniform workload. Assuming there are $k$ unique inserts and no secondary splits (because $k$ is small relative to $x_L$, the probability of this with a uniform workload is small), we have the following:

% \[ P[\text{node } i \text{ is split}] = 1 - \left( \frac{\frac{x_L}{p} - 1}{\frac{x_L}{p}} \right)^k \]
% \[ E[\text{split nodes}] = \frac{x_L}{p} - \frac{x_L}{p}\left(\frac{\frac{x_L}{p} - 1}{\frac{x_L}{p}}\right)^k \]

% We define $\alpha$ as the proportion of unique inserts in the upper levels of the LSM tree.  Thus, we know that the number of unique inserts is $k = \alpha x_{-L}$.  Using this, we have a total expected transition cost of:

% \begin{align*}
%     \text{Cost of transition} &= \left\lceil \frac{x_L}{p} \right\rceil + x_{-L}\left( \frac{1}{p} + 1\right) +  2\phi \frac{x_L}{p} \left(1 - \left( \frac{\frac{x_L}{p} - 1}{\frac{x_L}{p}} \right)^{\alpha x_{-L}} \right)  \\
%     &\quad\quad + \phi \left(\alpha x_{-L} - \frac{x_L}{p} \left( 1 - \left( \frac{\frac{x_L}{p} - 1}{\frac{x_L}{p}}\right)^{\alpha x_{-L}} \right) \right)
% \end{align*}

% Note that the second cost expression is a special case of the first one.  $\gamma$ is the proportion of entries in the upper levels of the LSM Tree that will cause a split in the B-Tree, and we can find $\gamma$ in terms of our other values (let $M = \frac{x_L}{p}$):
% \[ \gamma = \frac{M - (\frac{M-1}{M})^{\alpha x_{-L}}}{ x_{-L}} \]
% If we use this as our value for $\gamma$, then the two cost expressions are equivalent.  We use this fact to write a simpler expression of the transition cost:

% \[ \gamma = \frac{x_L - p(\frac{x_L-p}{x_L})^{\alpha x_{-L}}}{p x_{-L}}  \]

% \[ \text{Cost} = x_{-L}\left( \frac{1}{p} + 1 + \frac{x_L - p(\frac{x_L-p}{x_L})^{\alpha x_{-L}}}{p x_{-L}} 2 \phi + (1 - \frac{x_L - p(\frac{x_L-p}{x_L})^{\alpha x_{-L}}}{p x_{-L}})\phi \right) + \left\lceil \frac{x_L}{p} \right\rceil \]

% % \[\text{Cost of transition} = \left\lceil \frac{x_L}{p} \right\rceil +   x_{-L}\left( \frac{1}{p} + 1\right) +  2\phi\left(\frac{x_L}{p} - \frac{x_L}{p}\frac{(\frac{x_L}{p} - 1)^{\alpha x_{-L}}}{\frac{x_L}{p}}\right)  + \frac{(\frac{x_L}{p} - 1)^k}{\frac{x_L}{p}}\alpha\]


% \textbf{Preemptive Merge.}
% For the preemptive merge method of transitioning from an LSM Tree to a B-Tree, we assume that a proportion of $\alpha$ of the entries in the LSM Tree are not redundant/obsolete updates (and that $\frac{1}{\alpha}$ is the space amplification factor).  Thus, we can compute the cost of transitioning using this method:
% \[ \text{Cost} = \left( \sum_{k=1}^L \left\lceil \frac{x_k}{p} \right\rceil \right) (1 + \alpha \phi) \]
% To estimate the value of $\alpha$, we can use samples that we generate when merging runs in our natural LSM operations.  Whenever we merge two runs (whose total number of entries is $n_i$), we can keep track of the number of resulting entries after merging updates $m_i \leq n_i$.  If we have merged $k$ runs so far, we approximate $\alpha$ as follows by taking the average proportion of non-redundant entries:
% \[ \alpha \approx \frac{\sum_{i=1}^k m_i}{\sum_{i=1}^k n_i} \]

% Question: What to do about space amplification? How to estimate it? 

% Are our assumption in average case useful to look at? Should we look at other distributions?

% \textbf{Transition Model Plots.}
% To better understand how these transition cost models work, we plot the cost model of these transitions while varying the relative number of entries in the bottom level.  We vary $r$, the proportion of entries in the top levels of the LSM tree: $r = \frac{x_{-L}}{N}$.  We thus compute $x_{-L} = N r; \quad x_L = N (1-r)$ and plug these values into our cost models.  We plotted both the average case cost models as well as the worst case cost models below (for $p = 256; \phi=3; \alpha=0.8$):

% \begin{center}
% \includegraphics[scale=0.75]{preemptive_tradeoff.png}
% \end{center}

% This plot shows that for most values of $r$, preemptively merging is better.  Only for $r < .0025$ in the average case and $r < .0017$ in the worst case is using the "lowest level merge" faster.  However, we expect that if the entries of our LSM tree are large and not as many can fit in a page, then using the "lowest level merge" will be useful for more values of $r$.  We generate the same plot, this time with $p=2$ (which means that fewer entries fit in a page) to verify this intuition:

% \begin{center}
% \includegraphics[scale=0.75]{preemptive_tradeoff_2.png}
% \end{center}

% As expected, in this case using the lowest level of the LSM Tree in place is better for more values of $r$ than before.  

% \section{LSM to B-Tree: Incremental Merge Transition}

% \begin{center}
% \includegraphics[scale=0.1]{transition_graph.JPG}
% \end{center}

% We first considered modifying our LSM tree to incrementally increase the size ratio until it naturally merged into one level.  However, this method has no advantage over simply preemptively merging all the data because the final step in merging the LSM Tree will have to merge all of the data, which we could have done anyway via a preemptive merge.  As a result, we designed a method that avoids merging all of the data at once and instead incrementally merges data from the LSM Tree to build up the B-Tree from smallest values to largest values.  

% Each operation of this merge process generates $k$ pages of the lowest values in our LSM Tree, which we then write to the B-Tree.  We keep track of the minimum value of the data in the LSM Tree (which we denote $\theta$).  If an incoming query is looking for a key that is less than $\theta$, we direct the query to the B-Tree, and if the relevant key is greater than or equal to $\theta$, we direct the query to the LSM Tree.  This operation runs as follows:
% \begin{itemize}
%     \item We look at the first $k$ pages of each level in our LSM Tree
%     \item We sort-merge these pages to generate a sorted run of $k$ pages, which contains the lowest value in our LSM Tree
%     \item We append this run of $k$ pages to the end of the leaf level of our B-Tree, which we know is valid because we are guaranteed that all values in our B-Tree is less than $\theta$ and all values in our run are $\geq \theta$.
%     \item We update $\theta$ to be the new minimum value in our LSM Tree.
% \end{itemize}
% After we read pages from a level from disk, we keep the values in memory.  If these values become obsolete due to a merge occurring on the corresponding level, we simply update the values that we have stored in memory.  This does not incur any additional disk IO because we are writing the new merged values to disk during the process of the merge anyway, so we can keep these new values in memory at no additional disk IO cost.  This means that throughout the whole transition algorithm, our transition algorithm has to read all pages of the LSM Tree exactly once and write all values in our LSM Tree exactly once.  

% One thing that complicates this design is incoming updates.  We express time in terms of discrete \textit{steps}, which could be a second, minute, hour or greater which is a choice of the system admin.  Let $u$ be the number of insert updates per step in our workload, and the system can approximate $u$ by keeping track of updates over time. 

% Suppose we want to execute the transition in $M$ steps; there are $u$ updates per time step. Then, by the end of a transition, we will have a total of $N+Mu$ data.  To find an upper bound on the total cost of our transition algorithm, we assume that we have to move all of the data that we have by the end of the algorithm.  If the total amount of data we have to move is $N + Mu$, and the amount of data we move per step is $pk$, then the total number of steps is:
% \[\frac{N + Mu}{pk} = M\]
% We simplify this to get:
% \[M = \frac{N}{pk-u}\]
% This also shows that we can find $k$ as a function of $M$:
% \[ k = \frac{N + M u}{Mp} \]
% Each step of the algorithm has to read an average of $k$ pages and write exactly $k$ pages.  Thus, to cost one step, we have:
% \[C(\text{step})= k\phi + k = \frac{N + Mu}{Mp}(\phi + 1)\]
% \[  \frac{\partial}{\partial M}C(\text{step}) = \frac{-N}{M^2 p} (\phi + 1) \]
% This is decreasing with $M$, which suggests that we may be able to have lower average cost per step with this robust method.  Overall, we have to read and write every page of the data once, so the total cost of this algorithm is:
% \[ C(\text{overall}) = \frac{N + Mu}{p} (1 + \phi) \]
% Note that this is increasing with respect to $M$.  Thus, we can give $M$ as a parameter for the system admin which allows them to make the tradeoff between lower per-step cost and lower overall cost / time to transition.  

% Another useful way for a administrator to navigate this tradeoff is to allow her to specify a target step cost $\alpha$.  We can then find $M$ as a function of $\alpha$:
% \[ \alpha = \left(\frac{N + Mu}{Mp} \right) (\phi + 1) \to M = \frac{Np(\phi + 1)}{\alpha p - u (\phi + 1)} \]
% Thus, we can now use our computed $M$ to specify to the admin the overall transition cost and how long the transition will take.  This allows her to easily pick an $\alpha$ that will keep the transition from slowing down the system too much while also understanding how long the transition will take and its cost.  

% The overall memory usage of this algorithm will be $kp(L + 1)$ because we need to store $k$ pages for each level and an additional page for the output buffer, and each page has size $p$.  We express this in terms of $M$:
% \[ \text{Memory Usage} = \left(\frac{N}{M} + \frac{u}{p}\right)p(L + 1) \]
% This shows that increasing $M$ will also decrease the amount of memory that the transition algorithm requires.  This provides another metric by which the system admin can choose the optimal $M$.  


% We still need to figure out the details of how to incorporate updates into our system during transition. The optimal idea would seem to be to send updates less than the critical value to the B-Tree, and send those greater than the critical value to the LSM tree. So far, we have that at the $i$th step, $\frac{M - i}{M}u$ updates go to the LSM tree. How do you cost the updates here? $\frac{i}{M}$ updates go to the B-tree. For small $u$, we expect a split at almost every node, giving I/O of $1 + 2\phi$. For large $u$, the expected cost would be $1 + \phi(1 + \frac{1}{p})$.

% \subsection{Model Plots}
% We generated plots of our cost model using $N = 1,000,000$, $p=256$, $u=3$, and $\phi=1$.  Below is a plot of our algorithm's cost for each transition step as a function of $M$, the number of steps needed to complete the transition:

% \begin{center}
% \includegraphics[scale=0.75]{step_cost_varying_m.png}
% \end{center}

% We also allow the user to select a target step cost $\alpha$, and our algorithm will automatically select the appropriate $M$.  To show the effect of this choice of $\alpha$, we plot both $M$ and the total transition cost as a function of $\alpha$:

% \begin{center}
% \includegraphics[scale=0.75]{alpha_cost_and_time.png}
% \end{center}

% Note that, as expected, $M$ increases at a hyperbolic rate as $\alpha$ decreases ($M$ is similar to $\frac{1}{\alpha}$).  We also note that total transition cost is linear with respect to $M$, which makes sense because the amount of data that we need to transition increases by $u$ for each additional step that our algorithm takes.


% \textbf{Changing Number of Levels in LSM Tree.}
% We discuss another gradual merge process that could provide robustness to the transition process. In addition to transitioning an LSM tree to a B-tree, it may be valuable to be able to change the number of levels in the LSM tree.

% Increasing the number of levels seems rather trivial; for almost free, we can break levels up, using the resulting levels as new levels in the LSM tree. We discuss now ideas to decrease the number of levels in the LSM tree.

% The basic idea to reduce the number of levels by $a$ is to merge the top $a + 1$ levels of the LSM tree. This will have a cost of $(s_0 + s_0T + \ldots s_0T^a)(1 + \phi)$. After choosing a new $T' > T$, we push parts of higher levels down, until no level has any overflow corresponding to the new $T'$ value.

% This latter step can be executed in a number of ways. The cost of these methods and choice of $T'$ may vary depending on the workload and distribution of data within the runs of the LSM tree. We try to provide some worst case guarantees and qualitative benefits of different methods. Since higher levels have less data, we will want to touch data in only these levels in our methods. In particular, we only have to touch the first $k$ runs, where $k$ is the minimum positive integer such that 

% \[  (x_0 + x_1 + \ldots + x_k) - (1 + T' + \ldots + T'^{k - a}) \leq 0\]

% In the worst case, this is the $k$ such that 
% \[  (1 + T + \ldots + T^{k}) - (1 + T' + \ldots + T'^{k - a}) \leq 0\]
% \[  \frac{T^{k + 1} - 1}{T - 1} - \frac{T'^{k - a + 1}}{T' - 1} \leq 0\]
% The reasoning behind this is that  with this $k$ value, we have enough space to rearrange these levels.

% The simplest method is to transition is to merge the first $k$ levels. In this case, the first $k - a$ levels at the top of the new LSM tree will be empty, and each of the below levels will satisfy the $T'$ fanout factor. This method gives us a cost of at most

% \[ \text{Cost of Transition} = (1 + \phi)\sum_{i = 0}^{k}\left\lceil\frac{x_i}{p}\right\rceil \]

% One may argue that in the above method $k$ may be too large, meaning that we are moving too much data. In particular, after merging the first $a$ levels together, each level may be overflowing past its required size by a rather small amount. Are there ways to merge smaller portions of these runs into lower levels? If so, our transition cost would be reduced, but top runs would not be empty, so they would fill up more quickly. We present two methods of doing this.

% First, we can merge the top $0 \leq l < k$ levels together. Then, choose some key values for $\alpha$ and $\beta$ and merge keys $a$ in the remaining top $k - l$ levels such that $\alpha \leq a \leq \beta$. If we choose the $\alpha$ and $\beta$ so that the $T'$ fanout factor is satisfied for each level, we can still satisfy fanout factor constraints, while engaging in fewer I/O operations. One side effect of this process is that some of our new levels will have $2$ tiers. This is because merging keys in the range $\alpha \leq a \leq \beta$ will leave a run of keys less than $\alpha$ and a run greater than $\beta$. This however is not very problematic because these runs span disjoint ranges. In other words, point queries can function the same way and range queries will only have to cope with a small number of more random accesses. If data is uniformly distributed, then using this $\alpha$ and $\beta$ key method should not touch that much data in the final step. 

% If the data in the levels is distributed in a particularly adversarial way, this method of using $\alpha$ and $\beta$ may touch a large portion of the $k - l$ levels; the method may devolve into just merging the $k$ levels. In order to reduce this, we may apply this trick to levels in pairwise fashion: to levels $1$ and $2$, then to levels $2$ and $3$, then to $3$ and $4$, etc. The reason this may be beneficial is that we can guarantee that there exist $\alpha$ and $\beta$ such that the proportion of level $i + 1$ that falls under in between these values is less than the corresponding proportion in level $i$. In other words, if level $1$ is too large by a factor of $20$ percent, then we can find a range $[\alpha, \beta]$ such that $20$ percent of level $1$ is in this range, but at most $20$ percent of level $2$ is in the range. By doing this for every pair of levels from level $1$ to $k$, we can once again produce the $T'$ fanout factor guarantee. 

% \subsection{Next Steps}

% \begin{itemize}
%     \item Model transitioning between variations of B-Trees and LSM Trees
%     \item More developed analysis of changing the number of levels in an LSM tree (i.e. more details as to when this is beneficial, and how to compute the cost and make an intelligent decision of when to switch)
%     \item Clear analysis of different types of data and how these types affect transition cost (e.g. do entries take up a small portion of a page, or multiple pages)
% \end{itemize}


